Geometric Scaling Laws for Axial Flux Permanent Magnet Motors in In-Wheel Powertrain Topologies

In this paper, we present geometric scaling models for axial flux motors (AFMs) to be used for in-wheel powertrain design optimization purposes. We first present a vehicle and powertrain model, with emphasis on the electric motor model. We construct the latter by formulating the analytical scaling laws for AFMs, based on the scaling concept of RFMs from the literature, specifically deriving the model of the main loss component in electric motors: the copper losses. We further present separate scaling models of motor parameters, losses and thermal models, as well as the torque limits and cost, as a function of the design variables. Second, we validate these scaling laws with several experiments leveraging high-fidelity finite-element simulations. Finally, we define an optimization problem that minimizes the energy consumption over a drive cycle, optimizing the motor size and transmission ratio for a wide range of electric vehicle powertrain topologies. In our study, we observe that the all-wheel drive topology equipped with in-wheel AFMs is the most efficient, but also generates the highest material cost.

==> def.tex <==
% ------ Leo and Rick ------
% Margin comments 
\ifmargincomments
\newcommand{\msmargin}[2]{{\color{red}#1}\marginpar{\color{red}\raggedright\footnotesize [MaS]:\\ #2}}
\else
\newcommand{\msmargin}[2]{#1}
\fi

% Track revisioin changes
\ifrev
\newcommand{\rev}[1]{{\leavevmode\color{blue}#1}}
\else
\newcommand{\rev}[1]{{\leavevmode#1}}
\fi



% --------------------------





%\newcommand{\flexbrac}[1]{\ifthenelse{\equal{#1}{} }{}{(#1)}}
%\newcommand{\flexcomma}[1]{\ifthenelse{\equal{#1}{} }{}{,#1}}
\newcommand{\flexbrac}[1]{\if\relax\detokenize{#1}\relax \else (#1) \fi}
\newcommand{\flexcomma}[1]{\if\relax\detokenize{#1}\relax \else ,#1 \fi}

\newcommand{\tstart}[1]{t_{\mathrm{s}\flexcomma{#1}}}
\newcommand{\tend}[1]{t_{\mathrm{e}\flexcomma{#1}}}
\newcommand{\schedulegraph}{G_\mathrm{s}}
\newcommand{\ppp}[1]{p_{\mathrm{pp}} \flexbrac{#1}}
\newcommand{\pa}[1]{p_{\mathrm{a}} \flexbrac{#1}}
\newcommand{\pchtot}[1]{p_{\mathrm{ch,tot}} \flexbrac{#1}}
\newcommand{\pchtotrouted}[1]{p_{\mathrm{ch,tot,routed}} \flexbrac{#1}}
\newcommand{\pch}[2]{p_{\mathrm{ch}\flexcomma{#1}} \flexbrac{#2}}
\newcommand{\chargedenergy}[1]{E_{\mathrm{ch}\flexcomma{#1}}}
\newcommand{\abs}[1]{\lvert #1 \rvert}
%\newcommand{\problemname}{AMoDRCPDP}
\newcommand{\tmax}{t_{\mathrm{simend}}}
\newcommand{\ptildepred}[2]{\tilde{p}_{\mathrm{pred}\flexcomma{#1}} \flexbrac{#2}}
\newcommand{\ppred}[2]{p_{\mathrm{pred}\flexcomma{#1}} \flexbrac{#2}}
%\newcommand{\ppred}[2]{p_{\mathrm{pred},#1}(#2)}
\newcommand{\einit}[1]{E_{\mathrm{init}\flexcomma{#1}}}
\newcommand{\Vr}{V_\mathrm{r}}
\newcommand{\Ar}{A_\mathrm{r}}
\newcommand{\Gr}{G_\mathrm{r}}
\newcommand{\As}{A_\mathrm{s}}
\newcommand{\Vs}{V_\mathrm{s}}
\newcommand{\Ast}{\As^\dagger}

\newcommand{\gd}{\bar{\partial}}
\newcommand{\dt}{\textnormal{d}t}
\newcommand{\deta}{\textnormal{d}\eta}
%\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\Upr}{{\mathop{\mathrm{Upr}}}}
\newcommand{\Sgn}{{\mathop{\mathrm{Sgn}}}}
%\newcommand{\h}{\mathop{\mathrm{H}}}
\newcommand{\prox}{{\mathop{\mathrm{prox}}}}
\newcommand{\T}{^{\mathop{\mathrm{T}}}}
\newcommand{\diag}{{\mathop{\mathrm{diag}}}}
%\newcommand{\mod}{{\text{mod}}}
%boldmath
%bold greek
\newcommand{\val}{\mbox{\boldmath $\alpha$}}
\newcommand{\vbe}{\mbox{\boldmath $\beta$}}
\newcommand{\vga}{\mbox{\boldmath $\gamma$}}
\newcommand{\vde}{\mbox{\boldmath $\delta$}}
\newcommand{\vep}{\mbox{\boldmath $\epsilon$}}
\newcommand{\vze}{\mbox{\boldmath $\zeta$}}
\newcommand{\vet}{\mbox{\boldmath $\eta$}}
\newcommand{\vth}{\mbox{\boldmath $\vartheta$}}
\newcommand{\vio}{\mbox{\boldmath $\iota$}}
\newcommand{\vka}{\mbox{\boldmath $\kappa$}}
\newcommand{\vla}{\mbox{\boldmath $\lambda$}}
\newcommand{\vmu}{\mbox{\boldmath $\mu$}}
\newcommand{\vnu}{\mbox{\boldmath $\nu$}}
\newcommand{\vxi}{\mbox{\boldmath $\xi$}}
\newcommand{\vpi}{\mbox{\boldmath $\pi$}}
\newcommand{\vrh}{\mbox{\boldmath $\rho$}}
\newcommand{\vsi}{\mbox{\boldmath $\sigma$}}
\newcommand{\vta}{\mbox{\boldmath $\tau$}}
\newcommand{\vup}{\mbox{\boldmath $\upsilon$}}
\newcommand{\vph}{\mbox{\boldmath $\varphi$}}
\newcommand{\vch}{\mbox{\boldmath $\chi$}}
\newcommand{\vps}{\mbox{\boldmath $\psi$}}
\newcommand{\vom}{\mbox{\boldmath $\omega$}}

\newcommand{\vvep}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\vvrh}{\mbox{\boldmath $\varrho$}}
\newcommand{\vvpi}{\mbox{\boldmath $\varpi$}}
\newcommand{\vvsi}{\mbox{\boldmath $\varsigma$}}
\newcommand{\vvph}{\mbox{\boldmath $\phi$}}
%bold capital greek
\newcommand{\vGa}{\mathbf \Gamma}
\newcommand{\vDe}{\mathbf \Delta}
\newcommand{\vTh}{\mathbf \Theta}
\newcommand{\vLa}{\mathbf \Lambda}
\newcommand{\vXi}{\mathbf \Xi}
\newcommand{\vPi}{\mathbf \Pi}
\newcommand{\vSi}{\mathbf \Sigma}
\newcommand{\vUp}{\mathbf \Upsilon}
\newcommand{\vPh}{\mathbf \Phi}
\newcommand{\vPs}{\mathbf \Psi}
\newcommand{\vOm}{\mathbf \Omega}
%capital greek slanted, MIT amsmath-package
\newcommand{\iGa}{\varGamma}
\newcommand{\iDe}{\varDelta}
\newcommand{\iTh}{\varTheta}
\newcommand{\iLa}{\varLambda}
\newcommand{\iXi}{\varXi}
\newcommand{\iPi}{\varPi}
\newcommand{\iSi}{\varSigma}
\newcommand{\iUp}{\varUpsilon}
\newcommand{\iPh}{\varPhi}
\newcommand{\iPs}{\varPsi}
\newcommand{\iOm}{\varOmega}
%bold latin
\newcommand{\va}{\mathbf a}
\newcommand{\vb}{\mathbf b}
\newcommand{\vc}{\mathbf c}
\newcommand{\vd}{\mathbf d}
\newcommand{\ve}{\mathbf e}
\newcommand{\vf}{\mathbf f}
\newcommand{\vg}{\mathbf g}
\newcommand{\vh}{\mathbf h}
\newcommand{\vi}{\mathbf i}
\newcommand{\vj}{\mathbf j}
\newcommand{\vk}{\mathbf k}
\newcommand{\vl}{\mathbf l}
\newcommand{\vm}{\mathbf m}
\newcommand{\vn}{\mathbf n}
\newcommand{\vo}{\mathbf o}
\newcommand{\vp}{\mathbf p}
\newcommand{\vq}{\mathbf q}
\newcommand{\vr}{\mathbf r}
%\newcommand{\vs}{\mathbf s}
\newcommand{\vt}{\mathbf t}
\newcommand{\vu}{\mathbf u}
\newcommand{\vv}{\mathbf v}
\newcommand{\vw}{\mathbf w}
\newcommand{\vx}{\mathbf x}
\newcommand{\vy}{\mathbf y}
\newcommand{\vz}{\mathbf z}
\newcommand{\eins}{\mathbf 1}
%bold capital latin
\newcommand{\vA}{\mathbf A}
\newcommand{\vB}{\mathbf B}
\newcommand{\vC}{\mathbf C}
\newcommand{\vD}{\mathbf D}
\newcommand{\vE}{\mathbf E}
\newcommand{\vF}{\mathbf F}
\newcommand{\vG}{\mathbf G}
\newcommand{\vH}{\mathbf H}
\newcommand{\vI}{\mathbf I}
\newcommand{\vJ}{\mathbf J}
\newcommand{\vK}{\mathbf K}
\newcommand{\vL}{\mathbf L}
\newcommand{\vM}{\mathbf M}
\newcommand{\vN}{\mathbf N}
\newcommand{\vO}{\mathbf O}
\newcommand{\vP}{\mathbf P}
\newcommand{\vQ}{\mathbf Q}
\newcommand{\vR}{\mathbf R}
\newcommand{\vS}{\mathbf S}
\newcommand{\vT}{\mathbf T}
\newcommand{\vU}{\mathbf U}
\newcommand{\vV}{\mathbf V}
\newcommand{\vW}{\mathbf W}
\newcommand{\vX}{\mathbf X}
\newcommand{\vY}{\mathbf Y}
\newcommand{\vZ}{\mathbf Z}
%calligraphic
\newcommand{\ca}{\mathcal{a}}
\newcommand{\cb}{\mathcal{b}}
\newcommand{\cc}{\mathcal{c}}
\newcommand{\cd}{\mathcal{d}}
\newcommand{\ce}{\mathcal{e}}
\newcommand{\cf}{\mathcal{f}}
\newcommand{\cg}{\mathcal{g}}
\newcommand{\ch}{\mathcal{h}}
\newcommand{\ci}{\mathcal{i}}
\newcommand{\cj}{\mathcal{j}}
\newcommand{\ck}{\mathcal{k}}
\newcommand{\cl}{\mathcal{l}}
\newcommand{\cm}{\mathcal{m}}
\newcommand{\cn}{\mathcal{n}}
\newcommand{\co}{\mathcal{o}}
\newcommand{\cp}{\mathcal{p}}
\newcommand{\cq}{\mathcal{q}}
%\newcommand{\cr}{\mathcal{r}}
\newcommand{\cs}{\mathcal{s}}
\newcommand{\ct}{\mathcal{t}}
\newcommand{\cu}{\mathcal{u}}
%\newcommand{\cv}{\mathcal{v}}
\newcommand{\cw}{\mathcal{w}}
\newcommand{\cx}{\mathcal{x}}
\newcommand{\cy}{\mathcal{y}}
\newcommand{\cz}{\mathcal{z}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
%fraktur
\newcommand{\frA}{\mathfrak{A}}
\newcommand{\frB}{\mathfrak{B}}
\newcommand{\frC}{\mathfrak{C}}
\newcommand{\frD}{\mathfrak{D}}
\newcommand{\frE}{\mathfrak{E}}
\newcommand{\frF}{\mathfrak{F}}
\newcommand{\frG}{\mathfrak{G}}
\newcommand{\frH}{\mathfrak{H}}
\newcommand{\frI}{\mathfrak{I}}
\newcommand{\frJ}{\mathfrak{J}}
\newcommand{\frK}{\mathfrak{K}}
\newcommand{\frL}{\mathfrak{L}}
\newcommand{\frM}{\mathfrak{M}}
\newcommand{\frN}{\mathfrak{N}}
\newcommand{\frO}{\mathfrak{O}}
\newcommand{\frP}{\mathfrak{P}}
\newcommand{\frQ}{\mathfrak{Q}}
\newcommand{\frR}{\mathfrak{R}}
\newcommand{\frS}{\mathfrak{S}}
\newcommand{\frT}{\mathfrak{T}}
\newcommand{\frU}{\mathfrak{U}}
\newcommand{\frV}{\mathfrak{V}}
\newcommand{\frW}{\mathfrak{W}}
\newcommand{\frX}{\mathfrak{X}}
\newcommand{\frY}{\mathfrak{Y}}
\newcommand{\frZ}{\mathfrak{Z}}
\newcommand{\fra}{\mathfrak{a}}
\newcommand{\frb}{\mathfrak{b}}
\newcommand{\frc}{\mathfrak{c}}
\newcommand{\frd}{\mathfrak{d}}
\newcommand{\fre}{\mathfrak{e}}
\newcommand{\frf}{\mathfrak{f}}
\newcommand{\frg}{\mathfrak{g}}
\newcommand{\frh}{\mathfrak{h}}
\newcommand{\fri}{\mathfrak{i}}
\newcommand{\frj}{\mathfrak{j}}
\newcommand{\frk}{\mathfrak{k}}
\newcommand{\frl}{\mathfrak{l}}
\newcommand{\frm}{\mathfrak{m}}
\newcommand{\frn}{\mathfrak{n}}
\newcommand{\fro}{\mathfrak{o}}
\newcommand{\frp}{\mathfrak{p}}
%\newcommand{\frq}{\mathfrak{q}}
\newcommand{\frr}{\mathfrak{r}}
\newcommand{\frs}{\mathfrak{s}}
\newcommand{\frt}{\mathfrak{t}}
\newcommand{\fru}{\mathfrak{u}}
\newcommand{\frv}{\mathfrak{v}}
\newcommand{\frw}{\mathfrak{w}}
\newcommand{\frx}{\mathfrak{x}}
\newcommand{\fry}{\mathfrak{y}}
\newcommand{\frz}{\mathfrak{z}}
%Natural, Integer, Rational and Real Numbers
\newcommand{\sN}{\mathbb{N}}
\newcommand{\sZ}{\mathbb{Z}}
\newcommand{\sQ}{\mathbb{Q}}
\newcommand{\sR}{\mathbb{R}}
%Bar
\newcommand{\bN}{\bar{N}}
\newcommand{\bT}{\bar{T}}
\newcommand{\bx}{\bar{x}}
\newcommand{\bu}{\bar{u}}
\newcommand{\bb}{\bar{b}}
\newcommand{\bk}{\bar{k}}
\newcommand{\bv}{\bar{v}}
\newcommand{\bd}{\bar{d}}
\newcommand{\bs}{\bar{s}}
\newcommand{\bS}{\bar{S}}
\newcommand{\bp}{\bar{p}}
%\newcommand{\dp}{\Delta p}
\newcommand{\by}{\bar{y}}
\newcommand{\cbY}{\bar{\mathcal{Y}}}
\newcommand{\bU}{\bar{U}}
\newcommand{\bB}{\bar{B}}
\newcommand{\bgamma}{\bar{\gamma}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hk}{\hat{k}}
\newcommand{\he}{\hat{\ve}}
\newcommand{\bH}{\bar{H}}
\newcommand{\bK}{\bar{K}}
\newcommand{\lH}{\textit{\b{H}}}
\newcommand{\s}{\sigma}
%\newcommand{\bs}{\bar{\sigma}}
\newcommand{\ls}{\b{$\sigma$}}
\newcommand{\Mod}{\text{mod}}
%Derivative
\newcommand{\ddt}{\frac{\textnormal{d}}{\textnormal{d}t}}
\newcommand{\dds}{\frac{\textnormal{d}}{\textnormal{d}s}}
\newcommand{\dtds}{\frac{\textnormal{d}t}{\textnormal{d}s}}
\newcommand{\one}{\mathbb{1}}
\newcommand{\zero}{\mathbb{0}}
\newcommand{\Pho}{P_\mathrm{home}}
\newcommand{\Pgo}{P_\mathrm{go}}
\newcommand{\Pe}{\vP^\mathrm{e}}
\newcommand{\kref}{k_\mathrm{ref}}
\newcommand{\kinf}{k_\mathrm{inf}}
\newcommand{\kpoor}{k_\mathrm{poor}}
\newcommand{\krich}{k_\mathrm{rich}}
\newcommand{\kwealthy}{k_\mathrm{wealthy}}
\newcommand{\vPpoor}{\vP_{\mathrm{poor}}}
\newcommand{\vPok}{\vP_{\mathrm{ok}}}
\newcommand{\vPrich}{\vP_{\mathrm{rich}}}
\newcommand{\vPwealthy}{\vP_{\mathrm{wealthy}}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\summe}[2]{\sum_{\scriptstyle\mathclap{#1}}^{\scriptstyle\mathclap{#2}}}
